Code Soliloquies for Accurate Calculations in Large Language Models

High-quality conversational datasets are crucial for the successful development of Intelligent Tutoring Systems (ITS) that utilize a Large Language Model (LLM) backend. Synthetic student-teacher dialogues, generated using advanced GPT-4 models, are a common strategy for creating these datasets. However, subjects like physics that entail complex calculations pose a challenge. While GPT-4 presents impressive language processing capabilities, its limitations in fundamental mathematical reasoning curtail its efficacy for such subjects. To tackle this limitation, we introduce in this paper an innovative stateful prompt design. Our design orchestrates a mock conversation where both student and tutorbot roles are simulated by GPT-4. Each student response triggers an internal monologue, or `code soliloquy' in the GPT-tutorbot, which assesses whether its subsequent response would necessitate calculations. If a calculation is deemed necessary, it scripts the relevant Python code and uses the Python output to construct a response to the student. Our approach notably enhances the quality of synthetic conversation datasets, especially for subjects that are calculation-intensive. Our preliminary Subject Matter Expert evaluations reveal that our Higgs model, a fine-tuned LLaMA model, effectively uses Python for computations, which significantly enhances the accuracy and computational reliability of Higgs' responses. Code, models, and datasets is available at https://github.com/luffycodes/Tutorbot-Spock-Phys.

==> figures/diag.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.34]{images/diag2.png}
    \caption{A new framework. Here we introduce our multi-turn prompt approach. 1) Not a single generation like SPOCK prompt, 2) Code Soliloquy. Grey block is the dotted circle.}
    \label{fig:tutorbot}
\end{figure*}

==> sections/introduction.tex <==
\input{figures/mock_con}

In the rapidly evolving domain of Natural Language Processing (NLP), the creation of high-quality chatbots using pre-trained Large Language Models (LLMs) is heavily reliant on conversational datasets as shown by Vicuna model \citep{vicuna2023}.
With advanced models like Generative Pretrained Transformer-4 (GPT-4) \citep{gpt4sparkai}, it is possible to generate such synthetic yet engaging conversations by designing creative prompts \citep{sonkar2023class}.
CLASS framework \citep{sonkar2023class} demonstrates the capacity of GPT-4 to synthesize meaningful interactions between a student and a tutorbot to train effective ITS systems.
However, this framework largely caters to subjects that circumvent calculation-intensive problems, such as biology.

Generating synthetic conversations for subjects like physics, which require complex calculations, presents a significant challenge.
This is primarily due to the limited mathematical capabilities of models like GPT-4.
For instance, ChatGPT and GPT-4 achieve only $55\%$ and $59\%$ accuracy respectively on three-digit by three-digit multiplication tasks, as reported by \citep{gptbadmath}.
This limitation makes the one-shot prompt design introduced in CLASS inadequate for generating holistic conversations in calculation-intensive subjects. 

Recognizing these limitations in GPT-4's mathematical capabilities, we have developed an innovative approach to generate synthetic student-tutor dialogues that incorporate accurate calculations.
Our solution is a multi-turn, stateful prompt design that leverages GPT-4 to simulate both student and tutorbot roles.
Central to this design is the unique incorporation of `code soliloquies', a novel concept that significantly enhances the dialogue's computational accuracy.
For every input from the GPT-4 emulated student, we initiate a soliloquy within the GPT-4 tutorbot – an internal dialogue hidden from the student. 
During  this soliloquy, GPT-tutorbot prompts itself to determine whether its next response necessitates any calculations.
If a calculation is required, it proceeds to script the necessary code and then utilizes the output from this code to generate an informed response to the student. 
Given that GPT-4 demonstrates a remarkable proficiency in writing code, we ingeniously utilize this strength in our design through the process of code soliloquy. 
This allows us to overcome GPT-4's calculation limitations, thereby significantly enhancing the quality of the synthetic dialogues, particularly for subjects that are calculation-intensive.

To demonstrate the efficacy of our stateful prompt design and the quality of the generated synthetic conversations, we introduce Higgs, a variant of the LLaMA-2-70b-chat base model \citep{llama2}, fine-tuned on the generated conversational dataset.
In order to test Higgs, we also developed a comprehensive evaluation protocol.
The evaluation measures the accuracy and computational reliability of Higgs' responses, particularly its proficiency in using Python for computations whenever necessary.
The results from preliminary SME evaluations are highly encouraging. 
Higgs exhibited an impressive ability to determine when Python computations were necessary in the conversation, and it consistently generated valid code.
Most notably, Higgs accurately verified student's calculations by leveraging Python code, underlining the utility of our approach in improving the computational reliability of LLMs.
These results demonstrate the potential of our stateful prompt design and generated mock conversations with code soliloquies in significantly enhancing the capabilities of LLMs, particularly in the context of calculation-intensive subjects. 
By fostering accuracy and computational reliability, our approach can transform LLMs into more effective and reliable educational tools.
Code, models, and datasets can be accessed \href{https://github.com/luffycodes/Tutorbot-Spock-Phys}{here}\footnote{\url{https://github.com/luffycodes/Tutorbot-Spock-Phys}}.
% \input{figures/diag}


==> sections/v0/old_eval_protocol.tex <==
\label{sec:eval_protocol}
\input{tables/eval}

Our evaluation protocol takes a comprehensive six-point approach that critically assesses the GPT-4 bot's functionality. This methodology enables us to measure the effectiveness and precision of the bot at leveraging Python during educational conversations accurately.

1. Python Usage Accuracy: We begin the evaluation by assessing if the bot accurately invokes Python for scenarios that require computational resolution. This highlights the GPT-4 bot's ability to recognize computational requirements.

2. Code Description Accuracy: The next phase focuses on the accuracy of code descriptions. It evaluates how effectively the bot translates the computation requirements into natural language descriptions, forming the basis for the Python code generation.

3. Code Compilation Success: We then test whether the generated Python code is syntactically correct and executable. This step measures the reliability of the bot-generated Python code to ensure it's error-free in structure.

4. Code Execution Correctness: The fourth metric assesses the execution of the Python code, examining whether the output aligns with the expected results based on the description. Results from successful executions demonstrate the bot's competence in correctly modelling computational requirements.

5. Tutorbot Response Quality: Following the Python execution, we evaluate how effectively the bot utilises the Python output. We check if the bot not only accurately interprets the Python output but also whether it cogently incorporates this understanding into its response to the student. This assesses the GPT-4 bot's capacity to use Python output in constructing contextually fitting responses.

6. Calculation Verification: Lastly, we evaluate the bot's ability to use Python in verifying the student's calculation-based answers. Checking whether the bot can accurately cross-verify student's calculations using Python and provide appropriate feedback helps assess its ability as a teaching aid.

This rigorous six-point protocol helps us comprehensively assess the GPT-4 bot's ability to invoke, generate and utilize Python computations effectively in an educational dialogue.

==> sections/v0/old_methodology.tex <==
%Generating conversations with code soliliques using stateful prompt design

In this section, we outline our proposed stateful prompt design, which enables the generation of synthetic student-tutorbot conversations.
Our unique approach leverages `code soliloquies' to conduct accurate calculations whenever necessary during these dialogues.

Our design employs two distinct prompts, allowing the GPT-4 model to emulate both student and tutorbot roles, thereby facilitating a dynamic conversation. 
While a straightforward approach might be to instruct the model to ‘act as a student/tutorbot and respond to the tutorbot/student’, we instead adopt a more sophisticated strategy inspired by the CLASS framework.

Specifically, we craft the prompts to guide the conversation flow optimally.
The student-specific prompt, detailed in appendix~\ref{app:student}, instructs GPT-student to generate inquiries and responses in a manner that simulates a real student.
The tutorbot-specific prompt contains guidelines encouraging the GPT-tutorbot to break down complex problems into manageable subproblems, aiding the student in reaching the final solution through these incremental steps. 
The prompt also ensures the bot provides regular hints and refrains from prematurely divulging complete answers.

The heart of our methodology is the intricate design of the tutorbot prompt. 
This design integrates a sequence of four distinct state-prompts, enabling an internal monologue - a feature we refer to as the 'code soliloquy'. 
This soliloquy represents the tutorbot's internal process of determining whether its reply to the student's query necessitates any form of calculation. 
The tutorbot steps through these states for each response to the student, ensuring an accurate and contextually appropriate dialogue.

Having established the context of our methodology, let's delve into each of these four states in detail to better understand the internal monologue of the tutorbot.

\begin{enumerate}
\item `Deciding State': This is the initial state that determines whether a calculation is required to form the GPT-tutorbot's response to the student.
The GPT-tutorbot model is prompted with a specific prompt designed for this state (refer to appendix ~\ref{app:deciding_state}).
The prompt instructs the model to output `Use Python' to decide whether to utilize Python for calculations. 
The model should output `yes' if the student provided a numerical answer that needs to be verified using Python, or if the model anticipates its subsequent response to be reliant on mathematical calculations. 
In scenarios not requiring calculations, the model should output `no'. 
If the output is `yes', the next prompt corresponds to the `Use Python State'. 
Otherwise, the conversational flow transitions to the `No Python State'. 
Throughout this process, python functionalities remain hidden from the student.

\item `Use Python State': If GPT-tutorbot model decides to use python, the model is then prompted using prompt specific to`Use Python State' (refer to appendix ~\ref{app:use_python_state}).
The prompt instructs the model to first output a natural language description of the desired calculation, and then generate the corresponding python code, enclosed within backticks and the `python' keyword for easy parsing.

\item `Received Python State': Post the execution of the python code from previous step, the final state of code soliloquy is reached.
The GPT-tutorbot model is prompted using the specific prompt for this state (refer to appendix ~\ref{app:received_python_state}).
The model is instructed to use the python output to assess the student's answer and provide suitable feedback.
If the student's answer is approximately close to the python output (using rounding for comparison), the model is instructed to approve the answer. 
Once this state is concluded, the GPT-tutorbot's response is relayed to the GPT-student model, and the GPT-tutorbot model resets to the `Deciding State'.

\item `No Python State': If the GPT-tutorbot concludes during the 'Deciding State' that there's no need for Python, it transitions to the `No Python State'.
The prompt specific to this state (refer to appendix ~\ref{app:no_python_state}) instructs the model to continue the conversation and respond to the student.
Once the GPT-tutorbot's response is relayed to the GPT-student model, the GPT-tutorbot model reverts to the `Deciding State'. 
\end{enumerate}

Thus, our unique stateful prompt design facilitates the creation of synthetic conversations where the tutorbot, though limited in mathematical calculations ability, can skillfully use python for computations to guide the conversation accurately.
This methodology significantly enhances the quality of synthetic dialogues, paving the way for the next crucial phase: training our model with these enriched dialogues. 
In the following section, we discuss how these synthetic conversations are used to fine-tune our Higgs model.
